Equipping Federated Graph Neural Networks with Structure-aware Group Fairness

Graph Neural Networks (GNNs) have been widely used for various types of graph data processing and analytical tasks in different domains. Training GNNs over centralized graph data can be infeasible due to privacy concerns and regulatory restrictions. Thus, federated learning (FL) becomes a trending solution to address this challenge in a distributed learning paradigm. However, as GNNs may inherit historical bias from training data and lead to discriminatory predictions, the bias of local models can be easily propagated to the global model in distributed settings. This poses a new challenge in mitigating bias in federated GNNs. To address this challenge, we propose $\text{F}^2$GNN, a Fair Federated Graph Neural Network, that enhances group fairness of federated GNNs. As bias can be sourced from both data and learning algorithms, $\text{F}^2$GNN aims to mitigate both types of bias under federated settings. First, we provide theoretical insights on the connection between data bias in a training graph and statistical fairness metrics of the trained GNN models. Based on the theoretical analysis, we design $\text{F}^2$GNN which contains two key components: a fairness-aware local model update scheme that enhances group fairness of the local models on the client side, and a fairness-weighted global model update scheme that takes both data bias and fairness metrics of local models into consideration in the aggregation process. We evaluate $\text{F}^2$GNN empirically versus a number of baseline methods, and demonstrate that $\text{F}^2$GNN outperforms these baselines in terms of both fairness and model accuracy.

==> tables/all_results_table.tex <==
\begin{table*}[t]
\label{tab:results_pokec}
\centering
\setlength{\tabcolsep}{2.6pt}  % reduce column spacing
% \resizebox{0.8\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
           &                       & \multicolumn{4}{c}{Pokec-z}                                                                                                       & \multicolumn{4}{c}{Pokec-n}                                                                                                       \\ \cmidrule(lr){3-6} \cmidrule(lr){7-10} 
Method     & FL                    & Accuracy(\%) $\uparrow$ & AUC(\%) $\uparrow$   & $\Delta_{\text{SP}}$ (\%) $\downarrow$ & $\Delta_{\text{EO}}$(\%) $\downarrow$  & Accuracy(\%) $\uparrow$ & AUC(\%) $\uparrow$   & $\Delta_{\text{SP}}$ (\%) $\downarrow$ & $\Delta_{\text{EO}}$(\%) $\downarrow$ \\ \midrule
FairGCN    & \xmark & $65.48\pm1.42 $              & $71.94\pm1.19$  & $4.83\pm2.17$                  & $4.46\pm2.90$                                                & $64.99\pm1.20$              & $68.52\pm 1.48$ & $3.09\pm2.69$                 & $7.34\pm3.55$                                               \\
FairVGNN   & \xmark & $64.04\pm2.23$              & $72.54\pm0.4$  & $5.83\pm2.3$                  & $6.8\pm1.27$                                                 & $64.42\pm1.2$               & $68.55\pm0.25$ & $4.64\pm1.07$                 & $3.79\pm1.38$                                               \\
EDITS      & \xmark & $64.33\pm1.1 $              & $69.39\pm0.98$ & $5.91\pm1.93$                 & $6.78\pm2.86$                                                & $62.43\pm1.54$              & $66.68\pm1.56$ & $5.84\pm4.26$                 & $6.62\pm5.43$                                                \\
FairAug    & \xmark & $67.26\pm0.52$              & $67.21\pm0.52$ & $5.11\pm2.13$                 & $5.2\pm2.14$                                                 & $\mathbf{67.22\pm0.26}$              & $64.36\pm0.41$ & $3.33\pm0.77$                 & $5.47\pm1.18$                                               \\
\midrule
FairAug$_{\text{+FL}}$ & \cmark & $64.62\pm0.65$              & $64.73\pm0.67$ & $4.01\pm0.28$                 & $3.98\pm0.51$                                                & $64.38\pm0.38$              & $62.45\pm0.47$ & $4.31\pm1.32$                 & $5.98\pm1.96$                                            \\
FairFed    & \cmark & $65.48\pm2.63$              & $69.72\pm2.7$  & $2.92\pm1.28$                 & $3.08\pm1.21$                                                & $61.16\pm2.46$               & $61.97\pm1.93$ & $2.66\pm1.20$                 & $3.69\pm2.95$                                                \\
% \midrule
% \ourmethod  & \cmark & $\mathbf{67.75\pm1.09}$              & $\mathbf{72.61\pm1.56}$ & $\mathbf{2.11\pm0.53}$                 & $\mathbf{2.31\pm1.06}$                                                & $\mathbf{67.8\pm0.53}$               & $\mathbf{68.8\pm0.96}$  & $\mathbf{1.98\pm0.68}$                 & $\mathbf{1.17\pm1.04}$  \\
\ourmethod  & \cmark & $\mathbf{68.17\pm0.19}$              & $\mathbf{73.47\pm0.52}$ & $\mathbf{1.66\pm1.02}$                 & $\mathbf{1.49\pm0.52}$                                                & $67.00\pm0.27$               & $\mathbf{69.62\pm1.34}$  & $\mathbf{0.85\pm0.31}$                 & $\mathbf{1.00\pm1.03}$  \\
% \ourmethod$_{1/|\intra-\inter|}$  & \cmark  & $66.86 \pm 0.96$       & $71.91 \pm 0.87$   & $1.94 \pm  1.24$              & $1.42 \pm 0.66$          
% % & $19.8404$ 
% & $65.99 \pm 1.13$ & $68.14 \pm 1.49$ & $1.34 \pm 0.91$ & $1.34 \pm 0.63$     \\
% \ourmethod$_{1-|\intra-\inter|}$ & \cmark & $66.33 \pm 0.97$       & $71.42 \pm 1.41$   & $1.75 \pm 1.33$              & $1.91 \pm 1.06$
% & $66.69 \pm 1.05$ & $68.79 \pm 0.68$ & $2.04 \pm 1.04$ & $2.33 \pm 1.96$
\bottomrule
%\ourmethod+SGC   & \cmark & $66.08\pm1.15$              & $70.45\pm0.52$ & $\mathbf{1.09\pm0.54}$                 & $\mathbf{0.78\pm1.21}$                                                & $65.82\pm1.05$              & $67.64\pm1.91$ & $\mathbf{0.73\pm0.55}$                 & $\mathbf{0.75\pm0.42}$                                                \\ \bottomrule
\end{tabular}
% }
\end{table*}









\begin{table*}[t]
\label{tab:results_pokec}
\centering
\setlength{\tabcolsep}{2.6pt}  % reduce column spacing
% \resizebox{0.8\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
           & \multicolumn{4}{c}{Pokec-z}                                                                                                       & \multicolumn{4}{c}{Pokec-n}                                                                                                       \\ \cmidrule(lr){2-5} \cmidrule(lr){6-9} 
Method     & Accuracy(\%) $\uparrow$ & AUC(\%) $\uparrow$   & $\Delta_{\text{SP}}$ (\%) $\downarrow$ & $\Delta_{\text{EO}}$(\%) $\downarrow$  & Accuracy(\%) $\uparrow$ & AUC(\%) $\uparrow$   & $\Delta_{\text{SP}}$ (\%) $\downarrow$ & $\Delta_{\text{EO}}$(\%) $\downarrow$ \\ \midrule
FairGCN    & $65.48\pm1.42 $              & $71.94\pm1.19$  & $4.83\pm2.17$                  & $4.46\pm2.90$                                                & $64.99\pm1.20$              & $68.52\pm 1.48$ & $3.09\pm2.69$                 & $7.34\pm3.55$                                               \\
FairVGNN   & $64.04\pm2.23$              & $72.54\pm0.4$  & $5.83\pm2.3$                  & $6.8\pm1.27$                                                 & $64.42\pm1.2$               & $68.55\pm0.25$ & $4.64\pm1.07$                 & $3.79\pm1.38$                                               \\
EDITS      & $64.33\pm1.1 $              & $69.39\pm0.98$ & $5.91\pm1.93$                 & $6.78\pm2.86$                                                & $62.43\pm1.54$              & $66.68\pm1.56$ & $5.84\pm4.26$                 & $6.62\pm5.43$                                                \\
FairAug    & $67.26\pm0.52$              & $67.21\pm0.52$ & $5.11\pm2.13$                 & $5.2\pm2.14$                                                 & $\mathbf{67.22\pm0.26}$              & $64.36\pm0.41$ & $3.33\pm0.77$                 & $5.47\pm1.18$                                               \\
\midrule
FairAug$_{\text{+FL}}$ & $64.62\pm0.65$              & $64.73\pm0.67$ & $4.01\pm0.28$                 & $3.98\pm0.51$                                                & $64.38\pm0.38$              & $62.45\pm0.47$ & $4.31\pm1.32$                 & $5.98\pm1.96$                                            \\
FairFed    & $65.48\pm2.63$              & $69.72\pm2.7$  & $2.92\pm1.28$                 & $3.08\pm1.21$                                                & $61.16\pm2.46$               & $61.97\pm1.93$ & $2.66\pm1.20$                 & $3.69\pm2.95$                                                \\
\ourmethod  & $\mathbf{68.17\pm0.19}$              & $\mathbf{73.47\pm0.52}$ & $\mathbf{1.66\pm1.02}$                 & $\mathbf{1.49\pm0.52}$                                                & $67.00\pm0.27$               & $\mathbf{69.62\pm1.34}$  & $\mathbf{0.85\pm0.31}$                 & $\mathbf{1.00\pm1.03}$  \\
\bottomrule
\end{tabular}
% }
\end{table*}

\begin{table*}[t]
\caption{Performance of \ourmethod\ and baselines (Pokec-z and Pokec-n datasets).}

\label{tab:results_pokec}
\centering
\setlength{\tabcolsep}{2.6pt}  % reduce column spacing
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
  \midrule
  \multicolumn{9}{c}{{\bf Global model performance}} \\
  \midrule
  \multirow{ 2}{*}{Method} & \multicolumn{4}{c}{Pokec-z} & \multicolumn{4}{c}{Pokec-n}   \\
\cmidrule(lr){2-9}
   & Accuracy(\%) $\uparrow$ & AUC(\%) $\uparrow$   & $\Delta_{\text{SP}}$ (\%) $\downarrow$ & $\Delta_{\text{EO}}$(\%) $\downarrow$  & Accuracy(\%) $\uparrow$ & AUC(\%) $\uparrow$   & $\Delta_{\text{SP}}$ (\%) $\downarrow$ & $\Delta_{\text{EO}}$(\%) $\downarrow$ \\ \midrule
FairAug$_{\text{+FL}}$ & $64.62\pm0.65$              & $64.73\pm0.67$ & $4.01\pm0.28$                 & $3.98\pm0.51$                                                & $64.38\pm0.38$              & $62.45\pm0.47$ & $4.31\pm1.32$                 & $5.98\pm1.96$                                            \\
FairFed    & $65.48\pm2.63$              & $69.72\pm2.7$  & $2.92\pm1.28$                 & $3.08\pm1.21$                                                & $61.16\pm2.46$               & $61.97\pm1.93$ & $2.66\pm1.20$                 & $3.69\pm2.95$                                                \\
\ourmethod  & $\mathbf{68.17\pm0.19}$              & $\mathbf{73.47\pm0.52}$ & $\mathbf{1.66\pm1.02}$                 & $\mathbf{1.49\pm0.52}$                                                & $\mathbf{67.00\pm0.27}$               & $\mathbf{69.62\pm1.34}$  & $\mathbf{0.85\pm0.31}$                 & $\mathbf{1.00\pm1.03}$  
  \\
\bottomrule
\end{tabular}
}
\end{table*}

